First Evidence of New Physics in b <--> s Transitions

We combine all the available experimental information on Bs mixing, including the very recent tagged analyses of Bs to J/Psi phi by the CDF and D0 collaborations. We find that the phase of the Bs mixing amplitude deviates more than 3 sigma from the Standard Model prediction. While no single measurement has a 3 sigma significance yet, all the constraints show a remarkable agreement with the combined result. This is a first evidence of physics beyond the Standard Model. This result disfavours New Physics models with Minimal Flavour Violation with the same significance.

==> arxivbib.tex <==
\bibitem{CKM} N.~Cabibbo,
  % ``Unitary Symmetry and Leptonic Decays,''
  Phys.\ Rev.\ Lett.\ {\bf 10}, 531 (1963);
  %% CITATION = PRLTA,10,531;%%
  M.~Kobayashi and T.~Maskawa,
  % ``CP Violation In The Renormalizable Theory Of Weak Interaction,''
  Prog.\ Theor.\ Phys.\ {\bf 49}, 652 (1973).
  %% CITATION = PTPKA,49,652;%%

\bibitem{mfv} R.~S.~Chivukula and H.~Georgi,
  % ``Composite Technicolor Standard Model,''
  Phys.\ Lett.\ B {\bf 188}, 99 (1987);
  %% CITATION = PHLTA,B188,99;%%
  L.~J.~Hall and L.~Randall,
  % ``Weak scale effective supersymmetry,''
  Phys.\ Rev.\ Lett.\ {\bf 65}, 2939 (1990);
  %% CITATION = PRLTA,65,2939;%%
  E.~Gabrielli and G.~F.~Giudice,
  % ``Supersymmetric corrections to epsilon'/epsilon at the leading
  % order in QCD and QED,''
  Nucl.\ Phys.\ B {\bf 433}, 3 (1995) [Erratum-ibid.\ B {\bf 507}, 549
  (1997)] [arXiv:hep-lat/9407029];
  %% CITATION = NUPHA,B433,3;%%
  M.~Ciuchini \textit{et al.},
  %``Next-to-leading {QCD} corrections to B --> X/s gamma in supersymmetry,''
  Nucl.\ Phys.\  B {\bf 534}, 3 (1998)
  [arXiv:hep-ph/9806308];
  %%CITATION = NUPHA,B534,3;%%
  A.~J.~Buras \textit{et al.},
  % ``Universal unitarity triangle and physics beyond the standard
  % model,''
  Phys.\ Lett.\ B {\bf 500}, 161 (2001) [arXiv:hep-ph/0007085];
  %% CITATION = PHLTA,B500,161;%%
  G.~D'Ambrosio \textit{et al.},
  % ``Minimal flavour violation: An effective field theory approach,''
  Nucl.\ Phys.\ B {\bf 645}, 155 (2002) [arXiv:hep-ph/0207036];
  %% CITATION = NUPHA,B645,155;%%
  A.~J.~Buras,
  % ``Minimal flavor violation,''
  Acta Phys.\ Polon.\ B {\bf 34}, 5615 (2003) [arXiv:hep-ph/0310208].
  %% CITATION = APPOA,B34,5615;%%

\bibitem{utfit} M.~Bona {\it et al.}  [UTfit Collaboration],
  % ``The 2004 UTfit Collaboration report on the status of the
  % unitarity triangle in the standard model,''
  JHEP {\bf 0507}, 028 (2005) [arXiv:hep-ph/0501199];
  %% CITATION = JHEPA,0507,028;%%
  M.~Bona {\it et al.}  [UTfit Collaboration],
  % ``The unitarity triangle fit in the standard model and hadronic
  % parameters from lattice QCD: A reappraisal after the measurements
  % of Delta(m(s)) and BR(B --> tau nu/tau),''
  JHEP {\bf 0610}, 081 (2006) [arXiv:hep-ph/0606167].
  %% CITATION = JHEPA,0610,081;%%

\bibitem{ckmfit} J.~Charles {\it et al.}  [CKMfitter Group],
  % ``CP violation and the CKM matrix: Assessing the impact of the
  % asymmetric B factories,''
  Eur.\ Phys.\ J.\ C {\bf 41}, 1 (2005) [arXiv:hep-ph/0406184].
  %% CITATION = EPHJA,C41,1;%%

\bibitem{bspeng} B.~Aubert {\it et al.}  [BABAR Collaboration],
  % ``Measurements of CP-violating asymmetries in B decays to omega
  % K0(S),''
  arXiv:hep-ex/0607101;
  %% CITATION = HEP-EX/0607101;%%
  % ``Observation of CP violation in B0 --> eta' K0 decays,''
  Phys.\ Rev.\ Lett.\ {\bf 98}, 031801 (2007) [arXiv:hep-ex/0609052];
  %% CITATION = PRLTA,98,031801;%%
  % ``Measurement of CP asymmetry in B0 --> K0(S) pi0 pi0 decays,''
  Phys.\ Rev.\ D {\bf 76}, 071101 (2007) [arXiv:hep-ex/0702010];
  %% CITATION = PHRVA,D76,071101;%%
  % ``Measurement of CP Asymmetries in B0 --> K0S K0S K0S Decays,''
  Phys.\ Rev.\ D {\bf 76}, 091101 (2007) [arXiv:hep-ex/0702046];
  %% CITATION = PHRVA,D76,091101;%%
  % ``Measurements of CP-Violating Asymmetries in the Decay
  % B0-->K+K-K0,''
  Phys.\ Rev.\ Lett.\ {\bf 99}, 161802 (2007) [arXiv:0706.3885
  [hep-ex]];
  %% CITATION = PRLTA,99,161802;%%
  % ``Measurement of the CP-Violating Asymmetries in B0 -> KS pi0 and
  % of the Branching Fraction of B0 -> K0 pi0,''
  Phys.\ Rev.\ D {\bf 77}, 012003 (2008) [arXiv:0707.2980 [hep-ex]];
  %% CITATION = PHRVA,D77,012003;%%
  % ``Time-dependent Dalitz Plot Analysis of B0 --> Ks pi+ pi-,''
  arXiv:0708.2097 [hep-ex];
  %% CITATION = ARXIV:0708.2097;%%
  K.~F.~Chen {\it et al.}  [Belle Collaboration],
  % ``Observation of time-dependent CP violation in B0 --> eta' K0
  % decays and improved measurements of CP asymmetries in B0 --> Phi
  % K0, K0(S) K0(S) K0(S) and B0 --> J/psi K0 decays,''
  Phys.\ Rev.\ Lett.\ {\bf 98}, 031802 (2007) [arXiv:hep-ex/0608039];
  %% CITATION = PRLTA,98,031802;%%
  K.~Abe {\it et al.}  [Belle Collaboration],
  % ``Measurements of time-dependent CP violation in B0 --> omega
  % K0(S), f0(980) K0(S), K0(S) pi0 and K+ K- K0(S) decays,''
  Phys.\ Rev.\ D {\bf 76}, 091103 (2007) [arXiv:hep-ex/0609006];
  %% CITATION = PHRVA,D76,091103;%%
  % ``Measurements of CP Violation Parameters in B0 -> Kspi0pi0 and B0
  % -> KsKs Decays,''
  arXiv:0708.1845 [hep-ex].
  %% CITATION = ARXIV:0708.1845;%%

\bibitem{deltas} M.~Beneke,
  % ``Corrections to sin(2beta) from CP asymmetries in B0 --> (pi0,
  % rho0, eta, eta', omega, Phi) K(S) decays,''
  Phys.\ Lett.\ B {\bf 620}, 143 (2005) [arXiv:hep-ph/0505075];
  %% CITATION = PHLTA,B620,143;%%
  G.~Engelhard, Y.~Nir and G.~Raz,
  % ``SU(3) relations and the CP asymmetry in B --> K(S) K(S) K(S),''
  Phys.\ Rev.\ D {\bf 72}, 075013 (2005) [arXiv:hep-ph/0505194];
  %% CITATION = PHRVA,D72,075013;%%
  H.~n.~Li, S.~Mishima and A.~I.~Sanda,
  % ``Resolution to the B --> pi K puzzle,''
  Phys.\ Rev.\ D {\bf 72}, 114005 (2005) [arXiv:hep-ph/0508041];
  %% CITATION = PHRVA,D72,114005;%%
  G.~Engelhard and G.~Raz,
  % ``Using SU(3) relations to bound the CP asymmetries in B --> K K K
  % decays,''
  Phys.\ Rev.\ D {\bf 72}, 114017 (2005) [arXiv:hep-ph/0508046];
  %% CITATION = PHRVA,D72,114017;%%
  G.~Raz,
  % ``Using SU(3) flavor to constrain the CP asymmetries in B --> P P,
  % V P, V V decays involving b --> s transitions,''
  arXiv:hep-ph/0509125;
  %% CITATION = HEP-PH/0509125;%%
  A.~R.~Williamson and J.~Zupan,
  % ``Two body B decays with isosinglet final states in SCET,''
  Phys.\ Rev.\ D {\bf 74}, 014003 (2006) [Erratum-ibid.\ D {\bf 74},
  03901 (2006)] [arXiv:hep-ph/0601214];
  %% CITATION = PHRVA,D74,014003;%%
  H.~n.~Li and S.~Mishima,
  % ``Penguin-dominated B --> P V decays in NLO perturbative QCD,''
  Phys.\ Rev.\ D {\bf 74}, 094020 (2006) [arXiv:hep-ph/0608277].
  %% CITATION = PHRVA,D74,094020;%%

\bibitem{review} L.~Silvestrini,
  % ``Searching for new physics in b --> s hadronic penguin decays,''
  Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf 57}, 405 (2007)
  [arXiv:0705.1624 [hep-ph]].
  %% CITATION = ARNUA,57,405;%%

\bibitem{localized} T.~Gherghetta and A.~Pomarol,
  % ``Bulk fields and supersymmetry in a slice of AdS,''
  Nucl.\ Phys.\ B {\bf 586}, 141 (2000) [arXiv:hep-ph/0003129];
  %% CITATION = NUPHA,B586,141;%%
  K.~Agashe, G.~Perez and A.~Soni,
  % ``Flavor structure of warped extra dimension models,''
  Phys.\ Rev.\ D {\bf 71}, 016002 (2005) [arXiv:hep-ph/0408134];
  %% CITATION = PHRVA,D71,016002;%%
  R.~Contino \textit{et al.},
  % ``Warped/Composite Phenomenology Simplified,''
  JHEP {\bf 0705}, 074 (2007) [arXiv:hep-ph/0612180].
  %% CITATION = JHEPA,0705,074;%%

\bibitem{NMFV} K.~Agashe \textit{et al.},
  % ``Next to minimal flavor violation,''
  arXiv:hep-ph/0509117.
  %% CITATION = HEP-PH/0509117;%%

\bibitem{df2gen} M.~Bona {\it et al.}  [UTfit Collaboration],
  % ``Model-independent constraints on Delta F=2 operators and the
  % scale of New Physics,''
  arXiv:0707.0636 [hep-ph].
  %% CITATION = ARXIV:0707.0636;%%

\bibitem{sacha} S.~Davidson, G.~Isidori and S.~Uhlig,
  % ``Solving the flavour problem with hierarchical fermion wave
  % functions,''
  arXiv:0711.3376 [hep-ph].
  %% CITATION = ARXIV:0711.3376;%%

\bibitem{guts} S.~Baek \textit{et al.},
  % ``Neutrino oscillation, SUSY GUT and B decay,''
  Phys.\ Rev.\ D {\bf 63}, 051701 (2001) [arXiv:hep-ph/0002141];
  %% CITATION = PHRVA,D63,051701;%%
  D.~Chang, A.~Masiero and H.~Murayama,
  % ``Neutrino mixing and large CP violation in B physics,''
  Phys.\ Rev.\ D {\bf 67}, 075013 (2003) [arXiv:hep-ph/0205111];
  %% CITATION = PHRVA,D67,075013;%%
  R.~Harnik \textit{et al.},
  % ``Atmospheric neutrinos can make beauty strange,''
  Phys.\ Rev.\ D {\bf 69}, 094024 (2004) [arXiv:hep-ph/0212180];
  %% CITATION = PHRVA,D69,094024;%%
  J.~Hisano and Y.~Shimizu,
  % ``GUT relation in neutrino induced flavor physics in SUSY SU(5)
  % GUT,''
  Phys.\ Lett.\ B {\bf 565}, 183 (2003) [arXiv:hep-ph/0303071].
  %% CITATION = PHLTA,B565,183;%%

\bibitem{utfitbasic} M.~Ciuchini {\it et al.},
  % ``2000 CKM-triangle analysis: A critical review with updated
  % experimental inputs and theoretical parameters,''
  JHEP {\bf 0107}, 013 (2001) [arXiv:hep-ph/0012308].
  %% CITATION = JHEPA,0107,013;%%

\bibitem{cfactors} J.~M.~Soares and L.~Wolfenstein,
  % ``CP violation in the decays B0 $\to$ Psi K(S) and B0 $\to$ pi+
  % pi-: A Probe for new physics,''
  Phys.\ Rev.\ D {\bf 47}, 1021 (1993);
  %% CITATION = PHRVA,D47,1021;%%
  T.~Goto, N.~Kitazawa, Y.~Okada and M.~Tanaka,
  %``Model independent analysis of B anti-B mixing and CP violation in B
  %decays,''
  Phys.\ Rev.\  D {\bf 53}, 6662 (1996)
  [arXiv:hep-ph/9506311];
  %%CITATION = PHRVA,D53,6662;%%
  N.~G.~Deshpande, B.~Dutta and S.~Oh,
  % ``SUSY GUTs contributions and model independent extractions of CP
  % phases,''
  Phys.\ Rev.\ Lett.\ {\bf 77}, 4499 (1996) [arXiv:hep-ph/9608231];
  %% CITATION = PRLTA,77,4499;%%
  J.~P.~Silva and L.~Wolfenstein,
  % ``Detecting new physics from CP-violating phase measurements in B
  % decays,''
  Phys.\ Rev.\ D {\bf 55}, 5331 (1997) [arXiv:hep-ph/9610208];
  %% CITATION = PHRVA,D55,5331;%%
  A.~G.~Cohen \textit{et al.},
  % ``B factory physics from effective supersymmetry,''
  Phys.\ Rev.\ Lett.\ {\bf 78}, 2300 (1997) [arXiv:hep-ph/9610252];
  %% CITATION = PRLTA,78,2300;%%
  Y.~Grossman, Y.~Nir and M.~P.~Worah,
  % ``A model independent construction of the unitarity triangle,''
  Phys.\ Lett.\ B {\bf 407}, 307 (1997) [arXiv:hep-ph/9704287].
  %% CITATION = PHLTA,B407,307;%%

\bibitem{dmsCDF} A.~Abulencia {\it et al.}  [CDF Collaboration],
  % ``Observation of B/s0 anti-B/s0 oscillations,''
  Phys.\ Rev.\ Lett.\ {\bf 97}, 242003 (2006) [arXiv:hep-ex/0609040].
  %% CITATION = PRLTA,97,242003;%%

\bibitem{ASLD0} V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  % ``Measurement of the charge asymmetry in semileptonic $B_s$
  % decays,''
  Phys.\ Rev.\ Lett.\ {\bf 98}, 151801 (2007) [arXiv:hep-ex/0701007].
  %% CITATION = PRLTA,98,151801;%%

\bibitem{ACHD0} V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  % ``Measurement of the CP-violation parameter of B0 mixing and decay
  % with p anti-p --> mu mu X data,''
  Phys.\ Rev.\ D {\bf 74}, 092001 (2006) [arXiv:hep-ex/0609014].
  %% CITATION = PHRVA,D74,092001;%%

\bibitem{ASLCDF} CDF Collaboration, CDF note 9015.

\bibitem{tauBsflavspec} D.~Buskulic {\it et al.}  [ALEPH
  Collaboration],
  % ``Study Of The B(S)0 Anti-B(S)0 Oscillation Frequency Using D(S)-
  % Lepton+ Combinations In Z Decays,''
  Phys.\ Lett.\ B {\bf 377}, 205 (1996);
  %% CITATION = PHLTA,B377,205;%%
  F.~Abe {\it et al.}  [CDF Collaboration],
  % ``Measurement of the $B_s0$ meson lifetime using semileptonic
  % decays,''
  Phys.\ Rev.\ D {\bf 59}, 032004 (1999) [arXiv:hep-ex/9808003];
  %% CITATION = PHRVA,D59,032004;%%
  P.~Abreu {\it et al.}  [DELPHI Collaboration],
  % ``Measurement of the B/s0 lifetime and study of B/s0 anti-B/s0
  % oscillations using D/s l events,''
  Eur.\ Phys.\ J.\ C {\bf 16}, 555 (2000) [arXiv:hep-ex/0107077];
  %% CITATION = EPHJA,C16,555;%%
  K.~Ackerstaff {\it et al.}  [OPAL Collaboration],
  % ``Measurements of the B/s0 and Lambda/b0 lifetimes,''
  Phys.\ Lett.\ B {\bf 426}, 161 (1998) [arXiv:hep-ex/9802002];
  %% CITATION = PHLTA,B426,161;%%
  V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  % ``A Precise measurement of the $B0_{s}$ lifetime,''
  Phys.\ Rev.\ Lett.\ {\bf 97}, 241801 (2006) [arXiv:hep-ex/0604046];
  %% CITATION = PRLTA,97,241801;%%
  CDF Collaboration, CDF note 7386;
  CDF Collaboration, CDF note 7757;
  E.~Barberio {\it et al.}  [HFAG],
  % ``Averages of b-hadron properties at the end of 2005,''
  arXiv:hep-ex/0603003;
  %% CITATION = HEP-EX/0603003;%%
  CDF Collaboration, CDF note 9203.

\bibitem{CDFTAGGED} T.~Aaltonen {\it et al.}  [CDF Collaboration],
  % ``First Flavor-Tagged Determination of Bounds on Mixing-Induced CP
  % Violation in Bs -> J/psi phi Decays,''
  arXiv:0712.2397 [hep-ex].
  %% CITATION = ARXIV:0712.2397;%%

\bibitem{D0TAGGED} V.~M.~Abazov {\it et al.}  [D0 Collaboration],
  % ``Measurement of $\boldmath {B_s0}$ mixing parameters from the
  % flavor-tagged decay $B0_s \to J/\psi \phi$,''
  arXiv:0802.2255 [hep-ex].
  %% CITATION = ARXIV:0802.2255;%%

\bibitem{UTNP1} M.~Bona {\it et al.}  [UTfit Collaboration],
  % ``The UTfit collaboration report on the status of the unitarity
  % triangle beyond the standard model. I: Model-independent analysis
  % and minimal flavour violation,''
  JHEP {\bf 0603}, 080 (2006) [arXiv:hep-ph/0509219].
  %% CITATION = JHEPA,0603,080;%%

\bibitem{UTNP2} M.~Bona {\it et al.}  [UTfit Collaboration],
  % ``The UTfit collaboration report on the unitarity triangle beyond
  % the standard model: Spring 2006,''
  Phys.\ Rev.\ Lett.\ {\bf 97}, 151803 (2006) [arXiv:hep-ph/0605213].
  %% CITATION = PRLTA,97,151803;%%


